A Sharp Blockwise Tensor Perturbation Bound for Orthogonal Iteration

In this paper, we develop novel perturbation bounds for the high-order orthogonal iteration (HOOI) [DLDMV00b]. Under mild regularity conditions, we establish blockwise tensor perturbation bounds for HOOI with guarantees for both tensor reconstruction in Hilbert-Schmidt norm $\|\widehat{\bcT} - \bcT \|_{\tHS}$ and mode-$k$ singular subspace estimation in Schatten-$q$ norm $\| \sin \Theta (\widehat{\U}_k, \U_k) \|_q$ for any $q \geq 1$. We show the upper bounds of mode-$k$ singular subspace estimation are unilateral and converge linearly to a quantity characterized by blockwise errors of the perturbation and signal strength. For the tensor reconstruction error bound, we express the bound through a simple quantity $\xi$, which depends only on perturbation and the multilinear rank of the underlying signal. Rate matching deterministic lower bound for tensor reconstruction, which demonstrates the optimality of HOOI, is also provided. Furthermore, we prove that one-step HOOI (i.e., HOOI with only a single iteration) is also optimal in terms of tensor reconstruction and can be used to lower the computational cost. The perturbation results are also extended to the case that only partial modes of $\bcT$ have low-rank structure. We support our theoretical results by extensive numerical studies. Finally, we apply the novel perturbation bounds of HOOI on two applications, tensor denoising and tensor co-clustering, from machine learning and statistics, which demonstrates the superiority of the new perturbation results.

==> for_compare/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


%%%%%%%%%%%%%%%%%%%%ARXIV-format-start
% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{algorithmic}
%\usepackage[bookmarks, colorlinks=true, plainpages = false, citecolor = blue,linkcolor=red,urlcolor = blue, filecolor = blue,pagebackref]{hyperref}

%\usepackage{algorithmic}
\usepackage{mathtools}
\usepackage{empheq}
\usepackage{amsfonts}
\usepackage{amsgen,amsmath,amstext,amsbsy,amsopn,amssymb,subfigure,stmaryrd,mathabx}
%\usepackage[dvips]{graphicx}
\usepackage{comment}
\usepackage{enumitem}
%\usepackage{natbib}
\usepackage{booktabs}
\usepackage{blkarray}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{url}
\usepackage{longtable}
\usepackage{multirow}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
\DeclareGraphicsExtensions{.eps}
\fi

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\newtheorem{Example}{Example}  
\newtheorem{Definition}{Definition}
\newtheorem{Theorem}{Theorem}

\newtheorem{Lemma}{Lemma}
\newtheorem{Remark}{Remark}
\newtheorem{Corollary}{Corollary}
\newtheorem{Hypothesis}{Hypothesis}
\newtheorem{Proposition}{Proposition}
\newtheorem{Assumption}{Assumption}
\newtheorem{Condition}{Condition}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
	\newcommand{\eeas}{\end{eqnarray*}}

\newcommand {\reals}  {{\rm I \! R}}

\newcommand{\bbR}{\mathbb{R}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\Ra}{{\mathcal{R}}}
\newcommand{\Null}{{\mathcal{N}}}
\newcommand{\Range}{{\mathcal{R}}}

\newcommand{\0}{{\mathbf{0}}}
\newcommand{\1}{{\mathbf{1}}}
\renewcommand{\a}{{\mathbf{a}}}
\renewcommand{\b}{{\mathbf{b}}}
\renewcommand{\c}{{\mathbf{c}}}
\newcommand{\e}{{\mathbf{e}}}
\newcommand{\f}{{\mathbf{f}}}
\renewcommand{\u}{{\mathbf{u}}}
\renewcommand{\v}{{\mathbf{v}}}
\newcommand{\w}{{\mathbf{w}}}
\renewcommand{\r}{{\mathbf{r}}}
\newcommand{\x}{{\mathbf{x}}}
\newcommand{\y}{{\mathbf{y}}}
\newcommand{\z}{{\mathbf{z}}}
\newcommand{\X}{{\mathbf{X}}}
\newcommand{\B}{{\mathbf{B}}}
\newcommand{\J}{{\mathbf{J}}}
\newcommand{\E}{{\mathbf{E}}}
\newcommand{\C}{{\mathbf{C}}}
\newcommand{\D}{{\mathbf{D}}}
\renewcommand{\H}{{\mathbf{H}}}
\renewcommand{\L}{{\mathbf{L}}}
\newcommand{\I}{{\mathbf{I}}}
\newcommand{\M}{{\mathbf{M}}}
\renewcommand{\P}{{\mathbf{P}}}
\newcommand{\Q}{{\mathbf{Q}}}
\newcommand{\R}{{\mathbf{R}}}
\renewcommand{\S}{{\mathbf{S}}}
\newcommand{\U}{{\mathbf{U}}}
\newcommand{\V}{{\mathbf{V}}}
\newcommand{\W}{{\mathbf{W}}}
\newcommand{\Var}{{\rm Var}}
\newcommand{\Corr}{{\rm Corr}}
\newcommand{\Cov}{{\rm Cov}}
\newcommand{\A}{{\mathbf{A}}}
\newcommand{\Y}{{\mathbf{Y}}}
\newcommand{\Z}{{\mathbf{Z}}}
\newcommand{\T}{{\mathbf{T}}}
\newcommand{\F}{{\mathbf{F}}}
\newcommand{\G}{{\mathbf{G}}}
\newcommand{\bPi}{{\mathbf{\Pi}}}
\newcommand{\bcX}{{\mathbfcal{X}}}
\newcommand{\bcL}{{\mathbfcal{L}}}
\newcommand{\bcM}{{\mathbfcal{M}}}
\newcommand{\bcA}{{\mathbfcal{A}}}
\newcommand{\bcY}{{\mathbfcal{Y}}}
\newcommand{\bcB}{{\mathbfcal{B}}}
\newcommand{\bcS}{{\mathbfcal{S}}}
\newcommand{\bcF}{{\mathbfcal{F}}}
\newcommand{\bcZ}{{\mathbfcal{Z}}}
\newcommand{\bcT}{{\mathbfcal{T}}}
\newcommand{\bcH}{{\mathbfcal{H}}}
\newcommand{\bcN}{{\mathbfcal{N}}}
\newcommand{\bcE}{{\mathbfcal{E}}}
\newcommand{\bcR}{{\mathbfcal{R}}}
\newcommand{\bcI}{{\mathbfcal{I}}}

\newcommand{\tX}{{\mathbf{\widetilde{X}}}}
\newcommand{\tu}{{\mathbf{\widetilde{u}}}}
\newcommand{\tv}{{\mathbf{\widetilde{v}}}}

\newcommand{\Proj}{P}

\newcommand{\bX}{{\mathbf{\bar{X}}}}
\newcommand{\by}{{\mathbf{\bar{y}}}}

\newcommand{\cR}{{\cal R}}
\newcommand{\cN}{{\cal N}}

\newcommand{\bgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bvarepsilon}{\boldsymbol{\varepsilon}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\Bphi}{\boldsymbol{\phi}}
\newcommand{\Bpsi}{\boldsymbol{\psi}}
\newcommand{\Bdelta}{\boldsymbol{\delta}}

\newcommand{\mean}{{\rm mean}}
\newcommand{\rank}{{\rm rank}}
\newcommand{\var}{{\rm var}}
\newcommand{\SSigma}{\boldsymbol{\Sigma}}
\newcommand{\tr}{{\rm tr}}
\newcommand{\CV}{\operatorname{\rm CV}}
\newcommand{\GCV}{\operatorname{\rm GCV}}
%\newcommand{\diag}{{\rm diag}}
\newcommand{\poly}{{\rm poly}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\Trun}{{\rm Trun}}
\newcommand{\SVD}{{\rm SVD}}
\newcommand{\rmvec}{{\rm vec}}
\newcommand{\Ky}{{\rm Ky}}
\newcommand{\tHS}{{\rm HS}}
\newcommand{\HOSVD}{{\rm T-HOSVD}}

\newcommand{\pnorm}[1]{{[\![}#1{]\!]}}
\newcommand{\plangle}{{\langle\!\langle}}
\newcommand{\prangle}{{\rangle\!\rangle}}
\newcommand{\argmin}{\mathop{\rm arg\min}}
\newcommand{\argmax}{\mathop{\rm arg\max}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\supp}{{\rm supp}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}

\newcommand{\vc}[3]{\overset{#2}{\underset{#3}{#1}}} 

\def\az#1{\textcolor{red}{#1}}
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\anru}[1]{{\textcolor{blue}{[Anru: #1]}}}
\newcommand{\yuetian}[1]{{\textcolor{blue}{[Yuetian: #1]}}}

\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother 
\allowdisplaybreaks
%%%%%%%%%%%%%%%%%%%%%ARXIV-format-end




% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Tensor Perturbation Bounds}{Yuetian Luo, Anru Zhang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A Sharp Blockwise Tensor Perturbation Bound for Tensor Power Iteration}% \thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
%\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
%  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
%\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
%  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
%\and Jane E. Smith\footnotemark[3]}

\author{Yuetian Luo\thanks{Department of Statistics, University of Wisconsin-Madison 
  (\email{anruzhang@stat.wisc.edu, yluo86@wisc.edu, raskutti@stat.wisc.edu}).}
\and Anru Zhang\footnotemark[1]}
%\and Garvesh Raskutti\footnotemark[1]
%\and Ming Yuan\thanks{Department of Statistics, Columbia University (\email{my2550@columbia.edu}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

